Parameter-Efficient Fine-Tuning with Discrete Fourier Transform

Low-rank adaptation~(LoRA) has recently gained much interest in fine-tuning foundation models. It effectively reduces the number of trainable parameters by incorporating low-rank matrices $A$ and $B$ to represent the weight change, i.e., $\Delta W=BA$. Despite LoRA's progress, it faces storage challenges when handling extensive customization adaptations or larger base models. In this work, we aim to further compress trainable parameters by enjoying the powerful expressiveness of the Fourier transform. Specifically, we introduce FourierFT, which treats $\Delta W$ as a matrix in the spatial domain and learns only a small fraction of its spectral coefficients. With the trained spectral coefficients, we implement the inverse discrete Fourier transform to recover $\Delta W$. Empirically, our FourierFT method shows comparable or better performance with fewer parameters than LoRA on various tasks, including natural language understanding, natural language generation, instruction tuning, and image classification. For example, when performing instruction tuning on the LLaMA2-7B model, FourierFT surpasses LoRA with only 0.064M trainable parameters, compared to LoRA's 33.5M. Our code is released at \url{https://github.com/Chaos96/fourierft}.

==> table/bias.tex <==
\begin{table}[h!]
\centering
\caption{Results at different $f_c$. The best result for each of the three metrics is \textbf{bolded}, while the second best is \underline{underlined}.}
\label{tab:bias}
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{@{}l|cccccc|c@{}}
\toprule
$f_c$            & 0 & 100 & 200 & 300 & 400 & 480 & No bias \\ \midrule
Mean &  84.34  &   84.77  &   86.23  &  \textbf{86.50}   &  84.17   &  84.21    &     \underline{86.32}    \\ \midrule
Median &  85.17 &  85.21   &  86.00   &  \textbf{86.42}   &  85.02   &  84.32   &     \underline{86.40}    \\ \midrule
Std.          & 1.94  &  1.65   &  \underline{0.84}   &  \textbf{0.90}   &  1.32   &  1.22   &   \underline{0.97}      \\ \bottomrule
\end{tabular}%
}
\end{table}

==> table/dart.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[h!]
\centering
\caption{Results on the DART dataset with GPT-2 models. The best performance is shown in \textbf{bold}.}
\label{tab:dart}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{@{}cl|r|ccc@{}}
\toprule
Model & Method & \begin{tabular}[c]{@{}l@{}}\# Trainable\\ Parameters\end{tabular} & BLEU$\uparrow$ & MET$\uparrow$ & TER$\downarrow$ \\ \midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}GPT-2\\ Medium\end{tabular}} & FF & 354M & 46.2 & 0.39 & 0.46 \\
 & $\text{Adpt}^{\text{L}}$ & 0.37M & 42.4 & 0.36 & 0.48 \\
 & $\text{Adpt}^{\text{L}}$ & 11M & 45.2 & 0.38 & 0.46 \\
 & LoRA & 0.35M & 47.1 & 0.39 & 0.46 \\
 & AdaLoRA & 0.35M & 46.8 & 0.39 & \textbf{0.44} \\
 & FourierFT & 0.048M & \textbf{47.3} & \textbf{0.41} & 0.48 \\ \midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}GPT-2\\ Large\end{tabular}} & FF & 774M & 47.0 & 0.39 & 0.46 \\
 & $\text{Adpt}^{\text{L}}$ & 0.88M & 45.7 & 0.38 & 0.46 \\
 & $\text{Adpt}^{\text{L}}$ & 23M & 47.1 & 0.39 & \textbf{0.45} \\
 & LoRA & 0.77M & \textbf{47.5} & 0.39 & \textbf{0.45} \\
 & AdaLoRA & 0.77M & 47.3 & \textbf{0.42} & 0.46 \\
 & FourierFT & 0.072 & 47.4 & 0.39 & \textbf{0.45} \\ \bottomrule
\end{tabular}%
}
\end{table}

==> table/e2e.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[t!]
\centering
\caption{Results with GPT-2 Medium and Large models on E2E tasks. We present the result from the final epoch. For all metrics, higher values indicate better performance. * indicates that the results are taken from prior works. Best results are shown in \textbf{bold}. }
\label{tab:e2e}
\addtolength{\tabcolsep}{-5pt}
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{@{}lrccccc@{}}
\toprule
\multicolumn{1}{l|}{\textbf{Method}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\# Trainable\\ Parameters\end{tabular}} & BLEU & NIST & METEOR & ROUGE-L & CIDEr \\ \midrule
\multicolumn{7}{c}{GPT-2 Medium}                                             \\ \midrule
\multicolumn{1}{l|}{FT*}        & \multicolumn{1}{r|}{354.92M} & 68.2 & 8.62 & 46.2 & 71.0 & 2.47 \\
\multicolumn{1}{l|}{$\text{Adpt}^{\text{L}}$*}         & \multicolumn{1}{r|}{0.37M}   & 66.3 & 8.41 & 45.0 & 69.8 & 2.40 \\
\multicolumn{1}{l|}{$\text{Adpt}^{\text{L}}$*}         & \multicolumn{1}{r|}{11.09M}  & 68.9 & 8.71 & 46.1 & 71.3 & 2.47 \\
\multicolumn{1}{l|}{$\text{Adpt}^{\text{H}}$*}         & \multicolumn{1}{r|}{11.09M}  & 67.3\textsubscript{$\pm$.6} & 8.5\textsubscript{$\pm$.07} & 46.0\textsubscript{$\pm$.2} & 70.7\textsubscript{$\pm$.2} & 2.44\textsubscript{$\pm$.01} \\
\multicolumn{1}{l|}{LoRA}      & \multicolumn{1}{r|}{0.35M}   & 68.9\textsubscript{$\pm$.3} & 8.76\textsubscript{$\pm$.06} & 46.6\textsubscript{$\pm$.1} & 71.5\textsubscript{$\pm$.1} & \textbf{2.53}\textsubscript{$\pm$.03} \\
\multicolumn{1}{l|}{\textbf{FourierFT}} & \multicolumn{1}{r|}{0.048M}   & \textbf{69.1}\textsubscript{$\pm$.1}  & \textbf{8.82} \textsubscript{$\pm$.05} & \textbf{47.0} \textsubscript{$\pm$.3} & \textbf{71.8} \textsubscript{$\pm$.1} & 2.51\textsubscript{$\pm$.02} \\ \midrule
\multicolumn{7}{c}{GPT-2 Large}                                              \\ \midrule
\multicolumn{1}{l|}{FT*}        & \multicolumn{1}{r|}{774.03M} & 68.5 & 8.78 & 46.0 & 69.9 & 2.45 \\
\multicolumn{1}{l|}{$\text{Adpt}^{\text{L}}$*}         & \multicolumn{1}{r|}{0.88M}   & 69.1\textsubscript{$\pm$.1} & 8.68\textsubscript{$\pm$.03} & 46.3\textsubscript{$\pm$.0} & 71.4\textsubscript{$\pm$.2} & 2.49\textsubscript{$\pm$.0} \\
\multicolumn{1}{l|}{$\text{Adpt}^{\text{L}}$*}         & \multicolumn{1}{r|}{23.00M}  & 68.9\textsubscript{$\pm$.3} & 8.70\textsubscript{$\pm$.04} & 46.1\textsubscript{$\pm$.1} & 71.3\textsubscript{$\pm$.2} & 2.45\textsubscript{$\pm$.02} \\
\multicolumn{1}{l|}{LoRA}      & \multicolumn{1}{r|}{0.77M}   & 70.1\textsubscript{$\pm$.3} & 8.83\textsubscript{$\pm$.02} & 46.8\textsubscript{$\pm$.2} & \textbf{72.0}\textsubscript{$\pm$.3} & 2.47\textsubscript{$\pm$.02} \\
\multicolumn{1}{l|}{\textbf{FourierFT}} & \multicolumn{1}{r|}{0.072M} & \textbf{70.2}\textsubscript{$\pm$.2} & \textbf{8.90}\textsubscript{$\pm$.02} & \textbf{47.0}\textsubscript{$\pm$.2} & 71.8\textsubscript{$\pm$.1} &  \textbf{2.50} \textsubscript{$\pm$.02} \\ \bottomrule
\end{tabular}%
}
\end{table}

==> table/llama-new.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{The average scores on MT-Bench and Vicuna, assessed by GPT-4 for the generated answers. \dag indicates updating the layers other than \texttt{lm\_head} with LoRA. Higher score is better.}
\label{tab:llama}
\addtolength{\tabcolsep}{-4pt}
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{@{}l|l|r|cc@{}}
\toprule
Model & Method & \begin{tabular}[c]{@{}r@{}}\# Trainable\\ Parameters\end{tabular} & MT-Bench & Vicuna \\ \midrule
\multirow{3}{*}{LLaMA1-7B} & LoRA^{\dag}      & 159.9M &  &  \\ 
& LoRA      & 33.5M &  &  \\ 
                           & \textbf{FourierFT} & 0.25M &  &  \\ \midrule
\multirow{3}{*}{LLaMA1-13B} & LoRA^{\dag}        & 250.3M &  &  \\ 
& LoRA      & 52.4M &  &  \\
                           & \textbf{FourierFT} & 0.31M &   &  \\ \midrule
\multirow{3}{*}{LLaMA2-7B} & LoRA^{\dag}      & 159.9M & 5.19\textsubscript{$\pm$.1} &  \\ 
& LoRA      & 33.5M & 5.20\textsubscript{$\pm$.3} &  \\ 
                           & \textbf{FourierFT} & 0.25M & 5.18\textsubscript{$\pm$.3} &  \\ \midrule
\multirow{3}{*}{LLaMA2-13B} & LoRA^{\dag}        & 250.3M & 5.77\textsubscript{$\pm$.2} &  \\
& LoRA      & 52.4M & 5.80\textsubscript{$\pm$.2} &  \\
                           & \textbf{FourierFT} & 0.31M & 5.82\textsubscript{$\pm$.3}  &  \\\bottomrule
\end{tabular}%
}
\end{table}

==> table/web.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[h!]
\centering
\caption{Results on the WebNLG dataset with GPT-2 models. The best performance is shown in \textbf{bold}.}
\label{tab:web}
\resizebox{0.55\textwidth}{!}{%
\begin{tabular}{cl|r|ccc}
\hline
Model & Method & \begin{tabular}[c]{@{}r@{}}\# Trainable\\ Parameters\end{tabular} & BLEU$\uparrow$ & MET$\uparrow$ & TER$\downarrow$ \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}GPT-2\\ Medium\end{tabular}} & FF & 354M & 46.5 & 0.38 & 0.53 \\
 & $\text{Adpt}^{\text{L}}$ & 0.37M & 50.2 & 0.38 & 0.43 \\
 & $\text{Adpt}^{\text{L}}$ & 11M & 54.9 & 0.41 & \textbf{0.39} \\
 & LoRA & 0.35M & 55.3 & 0.41 & \textbf{0.39} \\
 & AdaLoRA & 0.35M & 54.9 & \textbf{0.43} & 0.42 \\
 & \textbf{FourierFT} & 0.048M & \textbf{55.6} & 0.41 & \textbf{0.39} \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}GPT-2\\ Large\end{tabular}} & FF & 774M & 55.5 & 0.42 & 0.42 \\
 & $\text{Adpt}^{\text{L}}$ & 0.88M & 56.0 & 0.41 & 0.39 \\
 & $\text{Adpt}^{\text{L}}$ & 23M & \textbf{57.7} & \textbf{0.43} & 0.39 \\
 & LoRA & 0.77M & 57.0 & 0.42 & 0.38 \\
 & AdaLoRA & 0.77M & 57.3 & 0.38 & 0.38 \\
 & \textbf{FourierFT} & 0.072 & 57.2 & 0.42 & \textbf{0.36} \\ \hline
\end{tabular}%
}
\end{table}
